Bucketed Ranking-based Losses for Efficient Training of Object Detectors

Ranking-based loss functions, such as Average Precision Loss and Rank&Sort Loss, outperform widely used score-based losses in object detection. These loss functions better align with the evaluation criteria, have fewer hyperparameters, and offer robustness against the imbalance between positive and negative classes. However, they require pairwise comparisons among $P$ positive and $N$ negative predictions, introducing a time complexity of $\mathcal{O}(PN)$, which is prohibitive since $N$ is often large (e.g., $10^8$ in ATSS). Despite their advantages, the widespread adoption of ranking-based losses has been hindered by their high time and space complexities. In this paper, we focus on improving the efficiency of ranking-based loss functions. To this end, we propose Bucketed Ranking-based Losses which group negative predictions into $B$ buckets ($B \ll N$) in order to reduce the number of pairwise comparisons so that time complexity can be reduced. Our method enhances the time complexity, reducing it to $\mathcal{O}(\max (N \log(N), P^2))$. To validate our method and show its generality, we conducted experiments on 2 different tasks, 3 different datasets, 7 different detectors. We show that Bucketed Ranking-based (BR) Losses yield the same accuracy with the unbucketed versions and provide $2\times$ faster training on average. We also train, for the first time, transformer-based object detectors using ranking-based losses, thanks to the efficiency of our BR. When we train CoDETR, a state-of-the-art transformer-based object detector, using our BR Loss, we consistently outperform its original results over several different backbones. Code is available at https://github.com/blisgard/BucketedRankingBasedLosses

==> misc/old_tables/old_experiments.tex <==


\begin{table*}
    \centering
    \setlength{\tabcolsep}{0.25em}
    \footnotesize
    \caption{Comparison on Multi-stage Object Detectors with RSLoss and Bucketed RSLoss using COCO Dataset.}
    \label{tab:MultiStage}
    \begin{tabular}{|c|c|c||c|c|c|c|c|c|} \hline
    {Method}& {Backbone} & Num. of Epochs &AP $\uparrow$ & $\mathrm{AP_{50}} \uparrow$ & $\mathrm{AP_{75}} \uparrow$ & $T_{iter}\downarrow$  &$T_{epoch}\downarrow$ & $T_{total}\downarrow$ \\ \hline\hline 
    RS-R-CNN & ResNet-50 & 12&$39.4$ & 59.5& 43.0 & 0.60 & 90.03 & 1046.94\\ \hline
    Bucketed RS-R-CNN & ResNet-50 & 12&39.5 & 59.5 & 42.8 & 0.20 & 30.25 & 363.02 \\ \hline
    RS-R-CNN+ &ResNet-50& 12&40.6 & 61.3 & 43.9 & 0.62 & 90.04 & 1080.51 \\ \hline
    Bucketed RS-R-CNN+ & ResNet-50 &12& 40.8 &61.4&49.3 & 0.21 & 31.81 & 381.83 \\ \hline
    RS-R-CNN (with DCN)&ResNet-101 &36& 47.3& 67.4 & 51.2 & 0.90 & 394.78 & 4737.39 \\ \hline
    Bucketed RS-R-CNN (with DCN) &ResNet-101&36 & 47.7 & 67.8 & 51.5 &  0.46 & 203.91 &  2447.02\\ \hline
    RS-R-CNN+ (with DCN)&ResNet-101 &36& 47.7 & 68.2 & 51.9 & 0.90 & 130.75 & 4707.27 \\ \hline
    Bucketed RS-R-CNN+ (with DCN)&ResNet-101&36 & 47.7 & 67.9 & 52.1 & 0.49 & 215.92?? & 2591.15\\ \hline
    \end{tabular}
\end{table*}

%-------------------------------------------------------------------------
\subsubsection{One-stage Object Detectors}
For the experiments with one-stage object detectors, we simply substituted the loss function while maintaining the same learning rate (0.008) and configuration parameters as used by Oksuz et al. \cite{RSLoss}, to validate the effectiveness of our method.

Leveraging our tailored gradient adjustment method, we've secured Average Precision (AP) scores on par with RSLoss \cite{RSLoss}. As can be seen from Table \ref{tab:OneStage}, we've also managed to cut down the training time by about 2.3 times for ATSS \cite{ATSS} and nearly 1.9 times for PAA \cite{paa}. This efficiency boost narrows the gap with well-recognized score-based loss functions such as Focal Loss \cite{FocalLoss}. With BucketedRSLoss, we observe only a marginal increase in training time—approximately 1.1 times longer than Focal Loss \cite{FocalLoss} on both architectures—yet RS Loss \cite{RSLoss} and BucketedRSLoss achieves an improvement of roughly 0.5 AP.
\begin{table*}
    \centering
    \setlength{\tabcolsep}{0.25em}
    \footnotesize
    \caption{Bucketed RS-Loss outperforms RS-Loss significantly on average training time, achieves x2.3 faster training time on ATSS \cite{ATSS} and x1.8 faster training time on PAA \cite{paa}. All models use ResNet-50. Standard configuration of each detector is used and we only replaced the loss function. }
    \label{tab:OneStage}
    \begin{tabular}{|c|c||c|c|c|c|c|c|} \hline
    {Method}& {Backbone}&AP $\uparrow$ & $\mathrm{AP_{50}} \uparrow$ & $\mathrm{AP_{75}} \uparrow$ & $T_{iter} \downarrow$  & $T_{epoch} \downarrow$ & $T_{total} \downarrow$ \\ \hline\hline 
    AP-Loss - ATSS&  ResNet-50 & 38.1 & 58.2 & 41.0 & 0.38 & 56.17 & 675.11 \\ \hline
    Bucketed AP-Loss - ATSS (ours) &  ResNet-50 & 38.5 & 58.6 & 41.3 & 0.18 & 27.05 & 324.68  \\ \hline
      Focal Loss - ATSS&  ResNet-50 & 39.4 & 57.5 & 42.8 & 0.16 & 24.62 & 295.47 \\ \hline
     RS-Loss - ATSS & ResNet-50 & 39.8 & 58.9 & 42.6 & 0.43 & 62.89 & 754.69 \\ \hline
    Bucketed RS-Loss - ATSS (ours) & ResNet-50 & 39.8 & 58.8 & 42.9 & 0.18 & 27.13 & 325.60\\ \hline
    Focal Loss - PAA &  ResNet-50 & 40.7 & 58.8 & 44.5 & 0.32 & 47.18 & 566.22 \\ \hline
    RS-Loss - PAA &ResNet-50& 40.8 & 58.8 & 44.6 & 0.68 & 98.64 & 1183.79 \\ \hline
   Bucketed RS-Loss - PAA (ours) & ResNet-50 & 40.9 & 59.0 & 44.4 & 0.36 & 52.46 & 629.60 \\ \hline
    \end{tabular}
\end{table*}


\subsection{Experiments on Instance Segmentation}
In our experiments on instance segmentation, we employed Mask R-CNN models utilizing ResNet50 and ResNet101 backbones, training them on the COCO and LVIS datasets. In line with Oksuz et al. \cite{RSLoss}, we maintained the same architectural design choices as were used in Faster R-CNN.
\subsubsection{Multi-stage Instance Segmentation}
\noindent \textbf{COCO:} By integrating our method with Mask R-CNN models and trained on the COCO dataset, we have recorded a substantial reduction in training time, approximately a 2.25$\times$ decrease on the ResNet50 backbone and $2\times$ decrease on the ResNet101 backbone.
\begin{table*}
    \centering
    \setlength{\tabcolsep}{0.25em}
    \footnotesize
    \caption{Comparison on Multi-stage Instance Segmentation with RSLoss and Bucketed RSLoss using COCO Dataset.}
    \label{tab:MultiStageSegmentation}
    \begin{tabular}{|c|c|c|c|c||c|c|c|c|c|c|c|} \hline
    \multirow{2}{*}{Method}& \multirow{2}{*}{Backbone}& \multicolumn{3}{|c||}{Segmentation Performance}&\multirow{2}{*}{$\mathrm{AP_{box}}$}&  \multirow{2}{*}{$T_{iter} \downarrow$} &\multirow{2}{*}{$T_{epoch} \downarrow$} & \multirow{2}{*}{$T_{total} \downarrow$}  \\ \cline{3-5}
    &&AP $\uparrow$&$\mathrm{AP_{50}} \uparrow$&$\mathrm{AP_{75}} \uparrow$& & & &\\ \hline
    RS-Mask R-CNN & ResNet-50 & 36.3 & 57.2 & 38.8 & 40.1&0.67 & 98.06 & 1176.82 \\ \hline
    Bucketed RS-Mask R-CNN & ResNet-50 & 36.2 & 57.2 & 38.8 & 39.9&0.29 & 42.26 & 507.16 \\ \hline
    RS-Mask R-CNN+ &ResNet-50& 37.3 & 58.9 & 39.7 & 41.1&0.69 & 100.56 & 1206.75 \\ \hline
    Bucketed RS-Mask R-CNN+ & ResNet-50 & 37.3 & 58.9 & 40 &41.1 &0.31 & 45.50 &  546.06\\ \hline
    RS-Mask R-CNN & ResNet-101 &40.2 & 61.8 &43.5 & 44.7&0.71 & 103.38 & 3721.84 \\ \hline
    Bucketed RS-Mask R-CNN & ResNet-101 & 40.3 & 62.0 & 43.8 & 44.7  & 0.33 & 47.97& 1727.02 \\ \hline
    RS-Mask R-CNN+ (with DCN) & ResNet-101 & 41.5 & 63.7 &  44.7 & 46.2 & 0.76&111.44 & 4012.16\\ \hline
    Bucketed RS-Mask R-CNN+ (with DCN) & ResNet-101 & 41.3 & 63.6 & 44.6 & 46.0 &0.38 & 57.50 & 2070.14  \\ \hline
    %RS-Mask R-CNN+ (with DCN) & ResNeXt-101 & &  &  &  &  &  &\\ \hline
    %Bucketed RS-Mask R-CNN+ (with DCN) & ResNeXt-101 & &  & & &  & &  \\ \hline
    \end{tabular}
\end{table*}
%-------------------------------------------------------------------------


\begin{table*}
    \centering
    \setlength{\tabcolsep}{0.25em}
    \footnotesize
\caption{Comparison on LVIS v1.0 val set. Models are trained with ResNet-50, multiscale images (range: $[640,800]$) for 12 epochs. 
%In addition, BAGS is finetuned for 12 epochs. 
\label{tbl:LVIS}}     \label{tab:MultiStageSegmentation}
    \begin{tabular}{|c|c||c|c|c|c|c|c|c|c|} \hline
    {Method}& {Backbone}&$\mathrm{AP_{mask}}$ $\uparrow$ & $\mathrm{AP_{r}} \uparrow$ & $\mathrm{AP_{c}} \uparrow$ &  $\mathrm{AP_{f}} \uparrow$ &$\mathrm{AP_{box}} \uparrow$ & $T_{iter} \downarrow$  & $T_{epoch} \downarrow$ & $T_{total} \downarrow$ \\ \hline 
    RFS+RS Loss & ResNet-50 &  &  &  &  & & 0.88  & 134.34 & 1612.15\\ \hline
    RFS+Bucketed RS Loss (ours) & ResNet-50 & & &  &  &  & 0.62 & 95.54 &  1146.49\\ \hline
    \end{tabular}
\end{table*}


%-------------------------------------------------------------------------

==> sec/_-TMP-3_background.tex <==

\section{Background}
%\section{Preliminaries and Background}

%In this section, we define the problem with a suitable notation and provide the necessary background for our approach by reviewing Average Precision Loss \cite{APLoss1,APLoss2} and Rank\&Sort Loss \cite{RSLoss}.
%In the context of object detection tasks, ranking-based loss functions offer significant advantages over score-based loss functions. These functions ease the process of hyperparameter tuning while directly optimizing the performance metric (AP). Ranking-based loss functions have proven to produce outstanding results in the field of various object detection and instance segmentation tasks, however it's crucial to acknowledge that they demand extensive training times due to their particular formulation.

%In their work on AP Loss, Chen et al. \cite{APLoss1,APLoss2} noted that the computational and memory complexity for AP Loss are notably greater than those of score-based losses such as Focal Loss and suffers from high complexity due to the necessity of computing pairwise differences. Similar to the AP Loss, RS Loss exhibits quadratic time complexity, leading to a noticeable increase in the time required for each training iteration, averaging 1.5 times longer in comparison.  To overcome this issue, our method replaces the sequential calculation of piecewise differences with a difference matrix through the implementation of a bucketing approach, resulting in a significant reduction in training time complexity.

\begin{comment}
\subsection{Problem Definition and Notation}

We have an object detection problem wherein we are interested in finding the class label $c_i \in \mathcal{C}$ and the bounding box coordinates $\mathbf{b}_i \in \mathbb{R}^4$ for each object $i$ in an input image. Given an image, an object detector generally provides many candidate object predictions where each prediction $i$ has an associated confidence score over classes $\mathbf{s}_i \in \mathbb{R}^{|\mathcal{C}|}$ in addition to the box coordinates $\mathbf{b}_i$.

An object detector is conventionally trained to minimize a weighted combination of a classification loss $\mathcal{L}_{cls}$ (e.g., Cross Entropy Loss \cite{FasterRCNN}, Focal Loss \cite{FocalLoss}) and a localization loss $\mathcal{L}_{loc}$ (e.g., Smooth-L1 Loss \cite{FasterRCNN}, Intersection-over-Union-based Losses \cite{GIoULoss}). During training in this conventional approach, each prediction is penalized based only on its closeness to its target.

Ranking-based approaches can be used for $\mathcal{L}_{cls}$ (e.g., in Average Precision Loss \cite{APLoss1,APLoss2}) or both $\mathcal{L}_{cls}$ and $\mathcal{L}_{loc}$ (in Rank\&Sort Loss \cite{RSLoss}). Unlike the conventional losses, ranking-based losses aim to rank the scores of positive detections above negative detections.
\end{comment}

\subsection{Revisiting Identity Update}% to Optimize Ranking-based Loss Functions}
Identity Update \cite{RSLoss} is a versatile method with well-defined steps to approximate the gradients of ranking-based loss functions, which, normally, do not have useful gradients.
%
The method assumes that a ranking-based loss function follows the particular form,
%
\begin{align}\scriptsize
\label{eq:LossIdentityUpdate}
\mathcal{L}= \frac{1}{Z}\sum \limits_{i \in \mathcal{P} \cup \mathcal{N}} (\ell(i) - \ell^*(i)), %\xRightarrow[\ell(i)\leftarrow 
\end{align}
%
in which $\mathcal{P}$ is the set of positive detections, $\mathcal{N}$ is the set of negative detections, $\ell(i)$ is the error computed on the $i$th detection, $\ell^*(i)$ is the target error (the lowest error possible) and $Z$ is the normalization constant.
%
To provide a simple example for more clarity, AP Loss \cite{APLoss1} can be defined by taking $\ell(i)$ as the precision error (1-precision) on $i$th positive example and $Z$ as $|\mathcal{P}|$ to average the precision errors: $\frac{1}{|\mathcal{P}|}\sum \limits_{i \in \mathcal{P} \cup \mathcal{N}} (\text{precision}(i) - \underbrace{\text{precision}^*(i)}_{\text{zero}})$.
%
The target error $\ell^*(i)$ ($\text{precision}^*(i)$) takes its lowest value as zero if the $i$th positive is ranked higher than all negatives; i.e., $\ell^*(i)$=1-precision=1-1=0. See Sect. \ref{sect:ap_loss} for more details.
%

Once formulated as in Eq. \ref{eq:LossIdentityUpdate}, Oksuz et al. \cite{RSLoss} showed that the loss can be computed and optimized by using the so-called primary terms \cite{APLoss1,APLoss2} as follows:
%
%Intuitively, a primary term, denoted by $L_{ij}$, defines the ranking error between a pair of logits $(s_i, s_j)$.
%
%In the following, we briefly revisit these two steps:

\noindent\textbf{1. Computation of the Loss.} For computing the loss $\mathcal{L}$ in Eq. \ref{eq:LossIdentityUpdate}, first, each pair of logits ($s_i$ and $s_j$) are compared by calculating their difference transforms as $x_{ij} = s_j - s_i$. $x_{ij}>0$ means that $s_j$ ranks higher than $s_i$. With a step function $H(\cdot)$, the number of detections higher than $s_i$ (and therefore its precision error) can be easily calculated (see Sect. \ref{sect:ap_loss}). Given  $x_{ij}$, the loss can be re-written and calculated in terms of  
primary terms $L_{ij}$ as 
$\mathcal{L} =\frac{1}{Z}\sum \limits_{i \in \mathcal{P} \cup \mathcal{N}}\sum \limits_{j \in \mathcal{P} \cup \mathcal{N} }  L_{ij}$, by taking:
%
\begin{align}
    \label{eq:PrimaryTermIdentityUpdate}
    L_{ij} = \left(\ell(i) - \ell^*(i) \right) p(j|i),
\end{align}
%
such that $p(j|i)$ is a probability mass function (pmf) that distributes the error computed on $i$th example over the $j$th example in order to determine the pairwise error term $L_{ij}$. $p(j|i)$ is commonly taken as a uniform distribution \cite{aLRPLoss,RSLoss}. Note that $ L_{ij}$ is non-differentiable since the step function ($H(\cdot)$) applied on $x_{ij}$ is non-differentiable, which will be discussed in Sect. \ref{sect:ap_loss}.

\begin{comment}Please note that the non-differentiability comes into play once the primary terms are obtained as this process involves the step function $H(\cdot)$. Following the common convention, we will assume that the step function is smoothed by $\delta$ resulting in:
\begin{equation}\footnotesize
\label{eq:h_smooth}
\small
H(x)=\left\{
\begin{aligned}
&0\, , & x < -\delta \\
&\frac{x}{2\delta}+0.5\, , & -\delta \leq x \leq \delta \\
&1\, , & \delta < x
\end{aligned}
\right.
\end{equation}
%
\end{comment}
%Then, the aim of the computation reduces to identifying the primary terms such that their normalized summation yields the same loss value $\mathcal{L}$ in Eq. \ref{eq:LossIdentityUpdate}.
%

\noindent\textbf{2. Optimization of the Loss.} Backtracking the steps of the loss computation, one can easily derive the gradients using the chain rule. However, the gradient of the primary term wrt. to the difference transform is non-differentiable. Denoting this term by $\Delta x_{ij}$, we have:
%
\begin{equation}\footnotesize
    \label{eq:Gradients}
    \frac{\partial \mathcal{L}}{\partial s_i} 
    = \sum \limits_{j,k} \frac{\partial \mathcal{L}}{\partial L_{jk}} \Delta x_{jk} \frac{\partial x_{jk}}{\partial s_i} 
    = \frac{1}{Z} \Big( \sum \limits_{j} \Delta x_{ji} - \sum \limits_{j} \Delta x_{ij} \Big). 
\end{equation}
%
Therefore, optimizing a ranking-based loss function reduces to determining $\Delta x_{ij}$. Inspired by Chen et al. \cite{APLoss1}, Oksuz et al. \cite{RSLoss} employ Perceptron Learning \cite{Rosenblatt} and show that $\Delta x_{ij}$ in Eq. \ref{eq:Gradients} is simply the primary term itself: $\Delta x_{ij}=-(L^*_{ij}-L_{ij})=-(0-L_{ij})=L_{ij}$, hence the name Identity Update. Plugging this into Eq. \ref{eq:Gradients} yields (see Oksuz et al. \cite{RSLoss} for the steps of the derivation):
%
\begin{equation}\footnotesize
    \label{eq:Final_Gradients}
    \frac{\partial \mathcal{L}}{\partial s_i} 
    = \frac{1}{Z} \Big( \sum \limits_{j} L_{ji} - \sum \limits_{j} L_{ij} \Big). 
\end{equation}
%
\textit{Therefore, both computing and optimizing the loss reduces determining the primary term $L_{ij}$}.

\subsection{Revisiting AP Loss and RS Loss from the Perspective of Identity Update}
\label{sect:ap_loss}

\noindent\textbf{AP Loss} \cite{APLoss1,APLoss2}. As aforementioned, AP Loss, as the average of the precision errors on positive examples, follows the form in Eq. \ref{eq:LossIdentityUpdate}.
%
Particularly, to see that, let us define AP Loss mathematically:
%
\begin{equation}\label{eq:ap_loss1}\footnotesize
\mathcal{L}_{AP} = 1-\mathrm{AP}=1-\frac{1}{|\mathcal{P}|} \sum_{i \in \mathcal{P}} \frac{\operatorname{rank}^{+}(i)}{\operatorname{rank}(i)}=\frac{1}{|\mathcal{P}|} \sum_{i \in \mathcal{P}} \frac{N_{FP}(i)}{\operatorname{rank}(i)},
\end{equation}
%
{\noindent}where $\operatorname{rank}^{+}(i)=\sum_{j\in \mathcal{P}} H(x_{ij})$ is the rank of the $i^{th}$ detection among positives whereas $\operatorname{rank}(i)=\sum_{j\in \mathcal{P}\cup\mathcal{N}} H(x_{ij})$ is the $i^{th}$ detection's rank among all detections; and $N_{FP}(i)$ is the number of false positives, i.e., the negatives ranked higher than $i$th positive: $N_{FP}(i)=\sum_{j\in \mathcal{N}} H(x_{ij})$. All these operations can easily defined by counting the score differences using the smoothed-step function: %pairwise relations $H(.)$: 
\begin{equation}\footnotesize
\label{eq:h_smooth}
\small
H(x)=\left\{
\begin{aligned}
&0\, , & x < -\delta \\
&\frac{x}{2\delta}+0.5\, , & -\delta \leq x \leq \delta \\
&1\, , & \delta < x
\end{aligned}
\right.
\end{equation}
%(Eq. \ref{eq:h_smooth}). As an example, $\operatorname{rank}(i)$ can be defined as:
%
%\begin{equation}\footnotesize
%    \operatorname{rank}(i) = \sum_{j\in \mathcal{P}\cup\mathcal{N}} H(x_{ij}).
%\end{equation}
%
Then, for defining AP Loss, the errors in Eq. \ref{eq:LossIdentityUpdate} can be derived as $\ell_{\mathrm{R}}(i)= \frac{N_{FP}(i)}{\operatorname{rank}(i)}$, $\ell^*_{\mathrm{R}}(i)=0$ and $Z=|\mathcal{P}|$.
%
Furthermore, defining $p_{R}(j|i)$ as a uniform pmf, that is $p_{R}(j|i) = \frac{\mathrm{H}(x_{ij})}{\mathrm{N_{FP}}(i)}$,  we can obtain the primary terms of AP Loss using Identity Update, completing the derivation for computation and optimization (Eq. \ref{eq:Final_Gradients}):
\begin{align}\footnotesize
    \label{eq:APPrimaryTermDefinition}
    L_{ij} = \begin{cases} \left(\ell_{\mathrm{R}}(i) - \ell^*_{\mathrm{R}}(i) \right) p_{R}(j|i), & \mathrm{for}\; i \in \mathcal{P}, j \in \mathcal{N} \\
    0, & \mathrm{otherwise},
    \end{cases}
\end{align}

\noindent\textbf{RS Loss} \cite{RSLoss}.  
In contrast to AP Loss, RS Loss includes an additional sorting objective ($\ell_S(i)$) in the loss function to promote better-localized positives to be ranked higher than other positives: 
\begin{align}\footnotesize
\label{eq:RSLoss}
    \mathcal{L}_\mathrm{RS} =\frac{1}{|\mathcal{P}|}\sum \limits_{i \in \mathcal{P}}  [ \underbrace{(\ell_{\mathrm{R}}(i)-\ell^*_{\mathrm{R}}(i))}_{\text{ranking}}
    +\underbrace{(\ell_{\mathrm{S}}(i)-\ell^*_{\mathrm{S}}(i))}_{\text{sorting}}],
\end{align}
The primary terms of RS Loss can be obtained in a similar manner to AP Loss (see the Supp.Mat. for derivations), yielding: %We do not delve into the details here, but only provide the resulting primary terms as follows:
\begin{align}\footnotesize\label{eq:RSPrimaryTermDefinition}
        L_{ij} = \begin{cases} \left(\ell_{\mathrm{R}}(i) - \ell^*_{\mathrm{R}}(i) \right) p_{R}(j|i), & \mathrm{for}\; i \in \mathcal{P}, j \in \mathcal{N} \\
        \left(\ell_{\mathrm{S}}(i) - \ell^*_{\mathrm{S}}(i) \right) p_{S}(j|i), & \mathrm{for}\;i \in \mathcal{P}, j \in \mathcal{P},\\
        0, & \mathrm{otherwise},
        \end{cases}
\end{align}
where %$\ell_{\mathrm{S}}(i)$ and $ \ell^*_{\mathrm{S}}(i)$ correspond to current and target sorting errors, and
$p_{S}(j|i)$ is the sorting pmf. Please note that RS Loss has exactly the same primary terms with AP Loss when $i \in \mathcal{P}, j \in \mathcal{N}$. The primary terms for $i \in \mathcal{P}, j \in \mathcal{P}$ directly targets promoting the better-localized positives.

\noindent\textbf{Complexity of Ranking-based Loss Functions.} 
These loss functions originally have the space complexity of \(\mathcal{O}((|\mathcal{P}|+|\mathcal{N}|)^2)\) \cite{APLoss1,APLoss2} as they need to compare each pair. This quadratic space complexity makes it infeasible compute these loss functions using modern GPUs as the number of logits in object detection is very large. To alleviate that, Chen et al.\cite{APLoss1} introduced two tricks at the expense of making the computation inefficient: (1) {Loop on Positives}: By implementing a loop over the positive examples, Chen et al. managed to reduce the time complexity to  \(\mathcal{O}(|\mathcal{P}|(|\mathcal{P}|+|\mathcal{N}|)) \approx \mathcal{O}(|\mathcal{P}||\mathcal{N}|)\) since $\mathcal{N}\gg \mathcal{P}$ and the space complexity to \(\mathcal{O}(|\mathcal{P}|+|\mathcal{N}|)\). (2) {Discard Trivial Negatives}: AP Loss considers negative examples with lower rank than all positives as trivial and disregards them. %that meet the condition $s_j - s_i \leq -\delta$ for all \(i \in \mathcal{P}\) and \(j \in \mathcal{N}\), categorizing these instances as trivial negative samples. %An additional process has been incorporated to identify and emphasize non-trivial examples. This may not lead to a significant improvement in speed during the initial stages of training, as almost all negative samples are non-trivial at that point. However, as the detector's performance improves,authors argued that the algorithm will gradually become faster.
%\end{enumerate}


\blockcomment{
Average Precision (AP) Loss \cite{APLoss1,APLoss2} formulates an objective for minimizing the AP:
%
\begin{equation}\label{eq:ap_loss1}
\small
\mathcal{L}_{AP} = 1-\mathrm{AP}=1-\frac{1}{|\mathcal{P}|} \sum_{i \in \mathcal{P}} \frac{\operatorname{rank}^{+}(i)}{\operatorname{rank}(i)}, 
\end{equation}
%
{\noindent}where $\mathcal{P}$ is the set of positive detections; $\operatorname{rank}^{+}(i)$ is the rank of the $i^{th}$ detection among positives whereas $\operatorname{rank}(i)$ is its rank among all detections. $\operatorname{rank}(i)$ can be defined with a simple counting operation (with $x_{ij} = s_j - s_i$):
%
\begin{equation}
    \operatorname{rank}(i) = \sum_{j\in \mathcal{P}\cup\mathcal{N}} H(x_{ij}),
\end{equation}
%
where $H(x)$ is 1 if $x>0$ and 0, otherwise. $\operatorname{rank}^{+}(i)$ can be defined similarly: $\operatorname{rank}^{+}(i) = \sum_{j\in \mathcal{P}} H(x_{ij})$. Plugging these definitions into Eq. \ref{eq:ap_loss1}, $\mathcal{L}_{AP}$ can be rewritten as:
%
\begin{equation}\label{eq:ap_loss2}
\small
\mathcal{L}_{AP} = \frac{1}{|\mathcal{P}|}\sum_{i\in \mathcal{P}} \sum_{j\in \mathcal{N}} \frac{H(x_{ij})}{\operatorname{rank}(i)} = \frac{1}{|\mathcal{P}|}\sum_{i\in \mathcal{P}} \sum_{j\in \mathcal{N}} L_{ij}, 
\end{equation}
%
{\noindent}where $L_{ij}$ is called the primary term. 
%Ranking task: Instead of employing a single box (anchor) with a score represented in a $C+1$ dimensional space, where $C$ denotes the number of classes, Chen et al. adopt a different approach. They replicate each box (anchor) $b_i$ $C$ times to create $b_{ik}$ instances, where $b_{ik}$ is accountable for the k'th class. Each of these instances possesses a scalar score denoted as $s_{ik}$ and is associated with a binary label $t_{ik}$, which can take one of three values: $1, 0, -1$. In the ranking task, the objective is to rank each positive box (where $t_{ik} = 1$) with higher scores $s_{ik}$ than all the negative boxes.

%\noindent\textbf{AP Loss Formulation} Recall that for each box $b_i$, there is a corresponding scalar score $s_i$ and a label $t_i$. Initially, they compute the pairwise differences with respect to every other box:
%\begin{equation}
%\small
%\forall i,j \  x_{ij} = s_j - s_i
%\end{equation}

%Next, the primary term of AP Loss is calculated as:
%    \begin{align}
%        \label{eq:GeneralPrimaryTermDefinition}
%        L_{ij} = \begin{cases}
%        \frac{\mathrm{H}(x_{ij})}{\mathrm{rank}(i)}, & \mathrm{for}\;i \in \mathcal{P}, j \in \mathcal{N} \\
%        0, & \mathrm{otherwise},
%        \end{cases}
%    \end{align}

%where \(H(\cdot)\) is the piecewise Heaviside step function:

\noindent\textbf{Optimization.} The AP Loss definitions in Eq. \ref{eq:ap_loss1} or \ref{eq:ap_loss2} are not differentiable. Chen et al. \cite{APLoss1,APLoss2} propose replacing the step function $H(\cdot)$ with an approximation: % $H_\delta(\cdot)$:
%
\begin{equation}
\label{eq:h_smooth}
\small
H(x)=\left\{
\begin{aligned}
&0\, , & x < -\delta \\
&\frac{x}{2\delta}+0.5\, , & -\delta \leq x \leq \delta \\
&1\, , & \delta < x
\end{aligned}
\right.
\end{equation}
%
The derivative of the loss with respect to the classification scores can be defined as follows using chain rule 
$\frac{\partial \mathcal{L}_{AP}}{\partial s_i} = \sum_{j,k} \frac{\partial\mathcal{L}_{AP}}{\partial L_{jk}} \Delta x_{jk} \frac{\partial x_{jk}}{\partial s_i}$. Chen et al. approximated $\Delta x_{ij}$ as $-L_{ij}\cdot \alpha_{ij}$ (with $\alpha_{ij}=1$ if $i\in \mathcal{P}$ and $j\in \mathcal{N}$) following the error-driven update in perceptron learning. 

%In order to address the issue of non-differentiability in ranking, AP Loss introduces a error-driven update mechanism that computes the gradient updates \( g_i \) for each predicted score \( s_i \) by utilizing the actual model outputs. For an input \( x_{ij} \), the update \( \Delta x_{ij} \) is derived as the difference between the optimal loss \( L^*_{ij} \) and the current loss \( L_{ij} \), denoted by:
%\begin{equation}
%\Delta x_{ij} = -(L^*_{ij} - L_{ij})    
%\end{equation}

%The AP-loss reaches its minimum value of 0 when \(L_{ij} \cdot y_{ij} = 0\). Hence, the update rule \( \Delta x_{ij} \) can be simplified to 
%\(
%\Delta x_{ij} = -L_{ij} \cdot y_{ij}
%\).
%And thus, the gradient \( g_i \) is computed as the negative sum of the products of loss terms and corresponding labels for both terms involving \( i \), yielding:
%\[
%\frac{\partial \mathcal{L}}{\partial s_i} = - \left( \sum_j L_{ji} \cdot y_{ji} + \sum_j L_{ij} \cdot y_{ij} \right)
%\]
%It accounts for the fact that the loss for positive examples (where \( y_{ij} = 1 \)) should contribute to the update, while for negative examples (where \( y_{ij} = 0 \)), the update is zero.



%This method enables the direct calculation of the partial derivatives \( \frac{\partial \mathcal{L}}{\partial s_i} \), where \( \mathcal{L} \) represents the loss function, thus facilitating the optimization process in ranking tasks. 









\subsection{Revisiting Rank \& Sort Loss}
\label{sect:rs_loss}
%-------------------------------------------------------------------------
Oksuz et al. \cite{RSLoss} extended AP Loss with a sorting-based objective that promotes a high-classification score ($s_i$) positive to have a high  Intersection over Union (IoU) value. To facilitate this, Oksuz et al. propose a formulation that can facilitate various forms of ranking and sorting objectives:
%AP Loss was introduced as a novel ranking-based technique tailored for one-stage detectors. Building on this foundational work, the RS Loss emerged as a versatile methodology, proving effective not only for one-stage object detection but also for multi-stage detectors and instance segmentation methods. Differing from AP Loss and other previous ranking-based approaches, RS Loss not only establishes a ranking where positives are prioritized above negatives but also organizes positive samples amongst themselves based on their continuous Intersection over Union (IoU) values. In addition to the AP Loss, RS loss incorporates an additional task, which is designed to arrange the scores $s_i$ in descending order with respect to continuous labels $y_i$(IoUs)  \(\in (0,1]\).
%
%AP Loss assigns a non-zero primary term only when \(i \in \mathcal{P}\) and \(j \in \mathcal{N}\), effectively disregarding the error between positive examples. However, these errors become particularly significant when dealing with continuous labels. In this context, the larger the label of \(i \in \mathcal{P}\), the larger $s_i$ should be, indicating a relationship between the label and the score.
%
%Oksuz et. al. redefine the RS Loss as the average of the differences between the current ($\ell_{\mathrm{RS}}(i)$) and target ($\ell_{\mathrm{RS}}^*(i)$) RS errors over positives (i.e. $y_i > 0$):
\begin{align}
\label{eq:RSLoss}
    \mathcal{L}_\mathrm{RS} =\frac{1}{|\mathcal{P}|}\sum \limits_{i \in \mathcal{P}}  \left( \ell_{\mathrm{RS}}(i)-\ell_{\mathrm{RS}}^*(i) \right),
\end{align}
where $\ell_{\mathrm{RS}}(i)$ is a sum of ranking error ($\ell_{\mathrm{R}}(i)$) and sorting error ($\ell_{\mathrm{S}}(i)$):  $\ell_{\mathrm{RS}}(i) = \ell_{\mathrm{R}}(i) + \ell_{\mathrm{S}}(i)$. The ranking error is simply a measure of precision, requiring comparisons between positives and negatives:
%
\begin{equation}\label{eq:ranking_error}
    \ell_{\mathrm{R}}(i) = \frac{\mathrm{N_{FP}}(i)}{\mathrm{rank}(i)} = \frac{\sum_{i\in \mathcal{P}}\sum_{j\in \mathcal{N}} H(x_{ij})}{\mathrm{rank}(i)},
\end{equation}
whereas the sorting error $\ell_{\mathrm{S}}(i)$ penalizes the ordering mismatch between classification score and IoU for positives:
%
\begin{align}
\label{eq:sorting_error}
    \ell_{\mathrm{S}}(i) = \frac{1}{\mathrm{rank^+}(i)}{\sum \limits_{j \in \mathcal{P}} {H}(x_{ij})(1-\textrm{IoU}_j)}. 
\end{align}
%
Oksuz et al. define the target error as follows: 
%take the target error for ranking (${\ell^*_{\mathrm{R}}(i)}$) to be zero while they define the target error for sorting as:
\begin{align}\scriptsize
\label{eq:RSTarget}
    \ell^*_{\mathrm{RS}}(i)= \underbrace{\cancelto{0}{\ell^*_{\mathrm{R}}(i)}}_{ \text{Target Ranking Error}}+ \underbrace{\frac{\sum \limits_{j \in \mathcal{P}} {H}(x_{ij})[\textrm{IoU}_j \geq \textrm{IoU}_i](1-\textrm{IoU}_j)}{\sum \limits_{j \in \mathcal{P}} {H}(x_{ij})[\textrm{IoU}_j \geq \textrm{IoU}_i]}}_{\ell^*_{\mathrm{S}}(i):\text{Target Sorting Error}}.
\end{align}
%
For \(i \in \mathcal{P}\), while the current ranking error represents the precision error, same as in AP Loss, and the current sorting error penalizes the positives with logits larger than $s_i$ by the average of their inverted labels, $1-\textrm{IoU}_j$. Note that when \(i \in \mathcal{P}\) is ranked above all \(j \in \mathcal{N}\), ${\mathrm{N_{FP}}(i)}$ is equal to 0, and the target ranking error, $\ell^*_R(i)$, is also 0 in this scenario.

With these definitions, the primary term for RS Loss can be defined as:
%
\begin{align}\footnotesize
        \label{eq:RSPrimaryTermDefinition}
        L_{ij} = \begin{cases} \left(\ell_{\mathrm{R}}(i) - \ell^*_{\mathrm{R}}(i) \right) p_{R}(j|i), & \mathrm{for}\; i \in \mathcal{P}, j \in \mathcal{N} \\
        \left(\ell_{\mathrm{S}}(i) - \ell^*_{\mathrm{S}}(i) \right) p_{S}(j|i), & \mathrm{for}\;i \in \mathcal{P}, j \in \mathcal{P},\\
        0, & \mathrm{otherwise},
        \end{cases}
    \end{align}

\noindent\textbf{Optimization.} Oksuz et al. \cite{RSLoss} extended the update mechanism of AP Loss and showed that the update \( \Delta x_{ij} \) can be simplified to \( L_{ij} \) for all examples. This yields to the following gradient as $\frac{\partial \mathcal{L}}{\partial s_i}$:
\begin{align}\footnotesize 
\label{eq:RSGradUpdate}
 \frac{1}{|\mathcal{P}|} \left( \ell^*_{\mathrm{R}}(i) - \ell_{\mathrm{R}}(i) + \sum \limits_{j \in \mathcal{P}} \left( \ell_{\mathrm{S}}(j) - \ell^*_{\mathrm{S}}(j) \right)  p_{\mathrm{S}}(i|j) \right).
\end{align}
%
\noindent\textbf{Complexity.} RS Loss also shares the same time and space complexity as AP Loss, which is \(\mathcal{O}(|\mathcal{P}|(|\mathcal{P}|+|\mathcal{N}|))\) and \(\mathcal{O}(|\mathcal{P}|+|\mathcal{N}|)\).

\section{Method: Bucketing Ranking-based Losses}
%-------------------------------------------------------------------------
%\subsection{Overview}

Our proposed method, Bucketed Ranking, aims to lower the high complexities of ranking-based losses (introduced in Sections \ref{sect:ap_loss} and \ref{sect:rs_loss} -- see also Table \ref{tab:comparative_summary}). Bucketed Ranking leverages the following observations (as summarized in Algorithm \ref{alg:bucketed_RS}): 
\begin{itemize}
    \item The number of negatives $\mathcal{|N|}$ is a prohibitive factor in these losses. For example, in Faster R-CNN \cite{FasterRCNN}, in the first epoch,  $\mathcal{|P|} \sim 5.10^2$ whereas $\mathcal{|N|} \sim 10^6$.

    \item As $\mathcal{|N|}$ is large, the positive-negative pair-wise comparisons (to obtain $L_{ij}$) and subsequent derivations cannot be stored as matrices in memory. Therefore, the ranking-based loss implementations use iterations, making them significantly slower compared to score-based losses (X vs Y minutes for the same detector, i.e., Faster R-CNN). 

    \item To improve efficiency, the way the comparisons are performed should be reconsidered. Since the goal in ranking is to rank positives above negatives, we find it helpful to group consecutively-scored negatives into buckets to obtain a set of buckets, $\mathcal{B}$. With this, positives can be compared with the buckets of negatives and since $|\mathcal{B}| \sim |\mathcal{P}| \ll |\mathcal{N}|$, complexity can be reduced significantly. This would also lower the memory costs, facilitating a matrix-based implementation.
\end{itemize}

%Both the AP Loss and the RS Loss have shown impressive performance on object detection tasks. However, a significant limitation associated with these ranking-based losses is the need for increased training time, especially when compared to score-based loss functions. It's widely acknowledged that the count of positive examples is considerably fewer than that of negative examples in visual detectors, $\mathcal{|P|}  \ll \mathcal{|N|}$. We observed that $\mathcal{|P|}$ + $\mathcal{|N|}$ is approximately $10^5$ and $10^6$ in one-stage and multi-stage detectors per image respectively where $\mathcal{|P|} \sim 5.10^2$ . Additionally,  Since ranking-based loss functions suppresses negatives over time, the number of relative negatives decreases significantly over time.

%Leveraging the insights from our observations, we reformulate the process: instead of the consecutive computation of pairwise differences, we remove the loop on positive indices and employ a difference matrix. To manage this matrix effectively and bypass the need for sequential calculations in paired scenarios—without incurring high memory costs—we introduce a bucketing strategy and achieve to a considerable decrease in the training time complexity. By using the mean value of consecutive negative scores, we generate a new bucketed representation for surrounding negative examples as one negative example  and reduce the total number of examples from $\mathcal{|P|}$ + $\mathcal{|N|}$ to $2 \times \mathcal{|P|}$ without any change in RS Loss formulation.

%-------------------------------------------------------------------------
\begin{algorithm}[t]
\small
\caption{AP Loss and RS Loss algorithms. Grey shows the additional operations of RS Loss compared to AP Loss.}
\begin{algorithmic}[1]
  \Require \(\{s_i\}\), predicted logits and \(\{t_i\}\), corresponding labels
  \Ensure \(\{g_i\}\), Gradient of loss wrt. input 

  \State $\forall i, \,\,\, g_i \gets 0$, $\mathcal{P} \gets \{i \mid t_i=1\}, \,\,\, \mathcal{N} \gets \{i \mid t_i=0\}$
  \State $s_{\text{min}} \gets \min_{i\in \mathcal{P}}\{s_{i}\}$, $\mathcal{\widehat{N}} \gets \{i\in \mathcal{N} \mid s_{i}> s_{\text{min}}-\delta\}$
  %\State $O \gets argsort(\{s_i \mid i\in \mathcal{P}\}) $ \Comment{Indexes of scores sorted in ascending order}

    \noindent \fcolorbox{red}{white}{%
  \begin{minipage}{\linewidth}

  \For{$i \in P$}
    \State \(\forall j\in \mathcal{P}\cup\mathcal{\widehat{N}}\), \(x_{ij}=s_j-s_i\) 
    \State \( \ell_{\mathrm{R}}(i) \) = $ N_{FP}(i) / rank(i) $ \Comment{\cref{eq:ranking_error}}
    \State \textcolor{gray}{$\forall j \in \mathcal{P}$, \( \ell_{\mathrm{S}}(j) \) and \( \ell_{\mathrm{S}}^{*}(j) \)} \Comment{ \cref{eq:sorting_error}, \cref{eq:RSTarget}}
    %\State $\forall j \in \mathcal{P}$ Compute \( \ell_{\mathrm{S}}^{*}(j) \)  \Comment{ \cref{eq:RSTarget}}
    \State $\forall j \in \mathcal{\widehat{N}}$, $L_{ij} = \ell_{\mathrm{R}}(i) \cdot p_{\mathrm{R}}(j|i)$
    \State \textcolor{gray}{$\forall j \in \mathcal{P}$, $L_{ij} = (\ell_{\mathrm{S}}(i) - \ell^*_{\mathrm{S}}(i)) \cdot  p_{\mathrm{S}}(j|i)$}
    \State $g_i \gets -\sum_{j\in \mathcal{\widehat{N}}} L_{ij} \textcolor{gray}{- \sum \limits_{j \in \mathcal{P}} L_{ij} + \sum \limits_{j \in \mathcal{P}} L_{ji}}$ \Comment{ \cref{eq:RSGradUpdate}}
    \State $\forall j \in \mathcal{\widehat{N}}, \,\,\, g_j \gets g_j+ L_{ij}$ \Comment{\cref{eq:RSGradUpdate}}
  \EndFor
    \end{minipage}%
}
  \State $\forall i, \,\,\, g_i \gets g_i / |\mathcal{P}|$ \Comment{Normalization}
  
\end{algorithmic}

\label{RSAlgorithm}
\end{algorithm}


\begin{algorithm}
\small
\caption{Bucketed RS and AP Losses. Grey shows the additional operations of BRS Loss compared to BAP Loss.}\label{alg:bucketed_RS}
\begin{algorithmic}[1]
\Require All scores \(\{s_i\}\) and corresponding labels \(\{t_i\}\) 
 \Ensure Gradient of input \(\{g_i\}\), ranking loss \( \ell_{\mathrm{R}} \), sorting loss \( \ell_{\mathrm{S}} \)
\State Sort logits to obtain \(\hat{s}_1\), \(\hat{s}_2\), $....$, \(\hat{s}_{|S|}\).
\State Bucket consecutive negative logits to obtain $B_1, ..., B_{|\mathcal{P}+1|}$.
\State Calculate \(\mathcal{X}_{pos}\)
\State Calculate \(\mathcal{X}_{neg}\)
\State $\forall i\in\mathcal{P}$, Calculate bucketed ranking error $\ell^b_\textrm{R}$ \Comment{\cref{eq:BRanking_Error}}.
\State \textcolor{gray}{Calculate IoU relations matrix $IoU_{rel}$}
\State \textcolor{gray}{Calculate current sorting error $\ell^{b}_{\mathrm{S}}$}  \Comment{\cref{eq:BCurrentSorting_Error}} 
\State \textcolor{gray}{Calculate target sorting error $\ell^{*b}_{\mathrm{S}}$} \Comment{\cref{eq:BTargetSorting_Error}}
\State \textcolor{gray}{Calculate sorting error \( \ell_{\mathrm{S}} \) = $\ell^{b}_{\mathrm{S}} - \ell^{*b}_{\mathrm{S}}$}
\State $\forall i, \,\,\, g_i \gets {\partial \mathcal{L}^b_{R}}/{\partial s_i} +  \textcolor{gray}{{\partial \mathcal{L}^b_{S}}/{\partial s_i}}$ \Comment{\cref{eq:bucketed_derivative}}
\State $\forall i, \,\,\, g_i \gets g_i / |\mathcal{P}|$ \Comment{Normalization}
\end{algorithmic}
\end{algorithm}





%-------------------------------------------------------------------------
\subsection{Bucketing Negatives for Reducing Complexity}


To identify the indices of sequential negative logits and bucket sizes for each bucket, the first step is to sort the logits, which is achieved using conventional methods. Let \( s_i \in S \) represent all logits ($\mathcal{P} \cup \mathcal{N}$) and \( t_i \in T \) represent all targets within a mini-batch. Let \(\hat{s}_1\), \(\hat{s}_2\), $....$, \(\hat{s}_{|S|}\) $\in \mathcal{S}$ be a sorted permutation of the logits such that  \(\hat{s}_1\) $\geq$  \(\hat{s}_2\) $\geq$  $....$ $\geq$ \(\hat{s}_{\mathcal{|S|}}\). Moreover, let us use $\hat{s}^+$ to denote a positive logit whereas $\hat{s}^-$ to denote a negative logit.

After sorting all logits w.r.t. their scores, we obtain buckets of negatives $B_1, ..., B_{|\mathcal{P}+1|}$ separated by positives:
%
\begin{align}
    \small
    B_1 \geq \hat{s}^+_1 \geq B_2 \geq \hat{s}^+_2 \geq ... \geq \hat{s}^+_{\mathcal{|P|}} \geq B_{|\mathcal{P}+1|}.
%    \underbrace{...}_{ \substack{\text{$b_1\geq 0$  } \\ \text{negative logits}}} \geq \hat{p}_1 \geq \underbrace{...}_{\substack{\text{$b_2\geq 0$  } \\ \text{negative logits}}} \geq \hat{p}_2 \geq ... \geq \hat{p}_{\mathcal{|P|}} \geq \underbrace{...}_{\substack{\text{$b_{|P|}\geq 0$  } \\ \text{negative logits}}}
\end{align}
%
In other words, we define \(\mathcal{|P|}\) buckets, each with sizes $b_1,b_2,…,b_{\mathcal{|P|}+1} \geq 0$, where $\sum_i b_i = \mathcal{|N|}$, and each bucket contains a sequence of negative logits in a sorted manner. 

We create a prototype of each bucket $B_i$ and replace the $b_i$ negative logits with a single logit $s^b_i$ by taking the mean over logits.  With this simplification, we attain a maximum of \( 2 \cdot |\mathcal{P}| \) logits. This ensures that within the sorted sequence, there are no consecutive negative examples. Using buckets, rather than individually computing each $x_{ij}$ for every $x \in \mathcal{P}$, we now efficiently derive \(\mathcal{X}_{pos}\)  with dimensions \(|\mathcal{P}| \times |\mathcal{P}|\) and \(\mathcal{X}_{neg}\) with dimensions \(|\mathcal{B}| \times |\mathcal{P}|\) as a matrix where  \(\mathcal{X}_{pos}\) is constituted by the column vectors $[x_{1j}, x_{2j}, \ldots, x_{|\mathcal{P}|j}]$ and \(\mathcal{X}_{neg}\) is constituted by the column vectors $[x_{1j}, x_{2j}, \ldots, x_{|\mathcal{B}|j}]$.

\noindent \textbf{Bucketed Ranking Error.} For simplicity, we follow the formulation of Oksuz et al. (\cite{RSLoss} and Section \ref{sect:rs_loss}). The ranking error in Eq. \ref{eq:ranking_error} requires the number of negatives above a certain positive $i$. 
%
%Recall that in ranking-based losses ranking error is computed as:    
%\begin{align}
%\label{eq:RSCurrent}
%    \ell_{\mathrm{R}}(i)= { \frac{\mathrm{N_{FP}}(i)}{\mathrm{rank}(i)}} , i \in \mathcal{P}.
%\end{align}
%
This implies that to compute the ranking error, we only require the sizes of the buckets (representing the sequence of negative logits preceding the positive logit for $i$) and the ranking order of the positive logits. With this, we can calculate $N_{\textrm{FP}}(i)$ as $\sum_{j=1}^i b_j$ and $\operatorname{rank}(i)$ as $\sum_{j=1}^i b_j + 1$. Using these in the definition of $\ell_{\mathrm{R}}(i)$ in Eq. \ref{eq:ranking_error}, we obtain the Bucketed Ranking Error as:
%
\begin{align}
\label{eq:BRanking_Error}
    \ell^{b}_{\mathrm{R}}(i)= { \frac{\sum_1^i b_i}{\sum_1^i (b_i +1)}} , \quad\quad i \in \mathcal{P}.
\end{align}
%

\noindent \textbf{Sorting Error.}  The sorting error in RS Loss (Eq. \ref{eq:sorting_error}) formulates constraints solely for positive logits. Thus, in the bucketed case, we merely need to transform the iterative calculations to matrix operations. Through straightforward transformations, this is achievable and demands a space complexity of \(\mathcal{O}(|\mathcal{P}|^2)\). \SK{Straightforward diye birakmayalim, denklemi ile matris halinde yazalim burayi}

In our transformation, in addition to \(\mathcal{X}_{pos}\)  and \(\mathcal{X}_{neg}\), we maintain the targets of the positive logits (IoUs) as a vector of size \(|\mathcal{P}|\) and also transform the IoU-relations as a matrix \(IoU_{rel}\) constructed with difference of IoU's for each positive logit, with dimension \(|\mathcal{P}| \times |\mathcal{P}|\).  Utilizing the matrices \(\mathcal{X}_{pos}\) and \(IoU_{rel}\), we are able to directly compute the current sorting loss  \(\ell^{b}_{\mathrm{S}}\) and target sorting loss \(\ell^{*b}_{\mathrm{S}}\) as:

%
\begin{align}
\label{eq:BCurrentSorting_Error}
    \ell^{b}_{\mathrm{S}}= { \frac{\sum (\mathcal{X}_{pos} \cdot ( 1 - IoU))}{\mathrm{rank^+}}} 
\end{align}
\begin{align}
\label{eq:BTargetSorting_Error}
    \ell^{*b}_{\mathrm{S}}= { \frac{\sum (\mathcal{X}_{pos} \cdot IoU_{rel} \cdot ( 1 - IoU))}{\sum (\mathcal{X}_{pos} \cdot IoU_{rel})}} 
\end{align}
%
 
\noindent\textbf{Optimization.} The gradient through Bucketed RS Loss ${\partial \mathcal{L}^b_{RS}}/{\partial s_i}$ can be calculated based on if $i\in \mathcal{P}$ or $i\in \mathcal{N}$:
%
\begin{align}\label{eq:bucketed_derivative}
\frac{\partial \mathcal{L}^b_\textrm{RS}}{\partial s_i} = \left\{
    \begin{aligned}
        &\frac{\partial \mathcal{L}_\textrm{RS}}{\partial s_i}, & i \in \mathcal{P} \\
        & \frac{\partial \mathcal{L}_\textrm{R}}{\partial {s}^b_i}\cdot\frac{1}{b_i} + \frac{\partial \mathcal{L}_\textrm{S}}{\partial s_i} , & i \in \mathcal{N} \\
    \end{aligned}
    \right.
\end{align}
where we use the gradients ${\partial \mathcal{L}_\textrm{RS}}/{\partial s_i}$ is as defined in RS Loss (Section \ref{sect:rs_loss});  ${\mathcal{L}_\textrm{RS}}/{\partial {s}^b_i}$ is calculated with respect to the mean logit of the bucket ${s}^b_i$ and distributed to each negative in the bucket equally with a factor of $1/b_i$. 

\subsection{Complexity of Bucketed Ranking TODO}

We will conduct a thorough analysis of complexity, taking into account both time and memory aspects.


\noindent\textbf{Removing the Loop on Positive Indices} 


\begin{itemize}
    \item Effect of sorting?
    \item When bucket numbers are equal to the number of positives/negative (there are no consecutive negative examples), then it corresponds to original RSLoss calculation. 
    \item When the number of buckets increases, the efficient algorithm approaches the RSLoss algorithm. Ideally, for P positive examples, there should be P buckets.
 

\end{itemize}

}
